Not Search, But Scan: Benchmarking MLLMs on Scan-Oriented Academic Paper Reasoning

With the rapid progress of multimodal large language models (MLLMs), AI already performs well at literature retrieval and certain reasoning tasks, serving as a capable assistant to human researchers, yet it remains far from autonomous research. The fundamental reason is that current work on academic paper reasoning is largely confined to a search-oriented paradigm centered on pre-specified targets, with reasoning grounded in relevance retrieval, which struggles to support researcher-style full-document understanding, reasoning, and verification. To bridge this gap, we propose \textbf{ScholScan}, a new benchmark for academic paper reasoning. ScholScan introduces a scan-oriented task setting that asks models to read and cross-check entire papers like human researchers, scanning the document to identify consistency issues. The benchmark comprises 1,800 carefully annotated questions drawn from nine error categories across 13 natural-science domains and 715 papers, and provides detailed annotations for evidence localization and reasoning traces, together with a unified evaluation protocol. We assessed 15 models across 24 input configurations and conducted a fine-grained analysis of MLLM capabilities for all error categories. Across the board, retrieval-augmented generation (RAG) methods yield no significant improvements, revealing systematic deficiencies of current MLLMs on scan-oriented tasks and underscoring the challenge posed by ScholScan. We expect ScholScan to be the leading and representative work of the scan-oriented task paradigm.

==> tables/comparison_of_dataset.tex <==
\begin{table*}[htbp]
  \centering
  \small
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{l c c c c c}
    \toprule
    \textbf{Benchmark} & \textbf{Mod.} & \textbf{Task P.} & \textbf{Eval.} &  \textbf{Cross-Evi.} \\
    \midrule
    \multicolumn{6}{l}{\textit{Document Understanding}} \\
    DocMath-Eval$_{\text{CompLong}}$ & T+TD & Search & A & 52.7 \\
    MMLongbench-Doc       & T+MD & Search & A & 33.7 \\
    LongDocURL            & T+MD & Search & A & 52.9 \\
    \midrule
    \multicolumn{6}{l}{\textit{Academic Paper Understanding}} \\
    CharXiv &  &  &  &  \\
    ArXivQA  &  &  &  &  \\
    MMCR    &  &  &  &  \\
    SCIQA   &  &  &  &  \\
    \midrule
    \textbf{ScholScan (ours)} & T+MD & Scan & A+P & 100\% \\
    \bottomrule
  \end{tabular}
  \caption{Reorganized comparison table schema. Cells intentionally left blank to be filled later.}
  \label{tab:benchmark_comparison}
\end{table*}

